GazeMotion: Gaze-guided Human Motion Forecasting

We present GazeMotion, a novel method for human motion forecasting that combines information on past human poses with human eye gaze. Inspired by evidence from behavioural sciences showing that human eye and body movements are closely coordinated, GazeMotion first predicts future eye gaze from past gaze, then fuses predicted future gaze and past poses into a gaze-pose graph, and finally uses a residual graph convolutional network to forecast body motion. We extensively evaluate our method on the MoGaze, ADT, and GIMO benchmark datasets and show that it outperforms state-of-the-art methods by up to 7.4% improvement in mean per joint position error. Using head direction as a proxy to gaze, our method still achieves an average improvement of 5.5%. We finally report an online user study showing that our method also outperforms prior methods in terms of perceived realism. These results show the significant information content available in eye gaze for human motion forecasting as well as the effectiveness of our method in exploiting this information.

==> discussion.tex <==
%------------------------------------------------------------------------
\section{Discussion}

\paragraph{Eye Gaze for Motion Forecasting}
Human eye gaze has been proven to be useful for many important VR/AR applications including interaction intent prediction~\cite{david2021towards}, task recognition~\cite{hu2022ehtask}, as well as cognitive load estimation~\cite{bozkir2019person}.
However, its effectiveness for human motion forecasting has not been explored yet.
We are the first to demonstrate that eye gaze is effective for human motion forecasting, achieving significantly better performances over the state of the art (Table \ref{tab:global} and Table \ref{tab:local}).
More importantly, we make a significant step forward by showing the potential of applying gaze prediction to improve the performances of motion forecasting methods (Table \ref{tab:ablation_gaze}).
With the rapid development of eye tracking technology, eye gaze information can be easily accessed in many commercial VR/AR devices such as HTC Vive Pro Eye, Varjo XR-4, and Hololens 2, paving the path for developing eye gaze-based applications.
Our gaze-guided motion forecasting method can be integrated into such devices to support many important VR/AR applications such as collision avoidance~\cite{zheng2022gimo}, redirected walking~\cite{sun2018towards}, and motor augmentation~\cite{lotti2020adaptive}.

%\paragraph{Improvements of Our Method}
%Through extensive experiments (Table \ref{tab:global} and Table \ref{tab:local}) and a user study (Section \ref{sec:user study}), we demonstrated that

\paragraph{Head Direction as a Proxy to Eye Gaze}
Considering that eye gaze information is not always available in VR/AR devices, we proposed to use head direction, which can be easily accessed in VR/AR headsets, as a proxy to eye gaze.
Extensive experiments demonstrated that head direction can effectively guide human motion forecasting, achieving significantly better performances over the state of the art (Section \ref{sec:head}). 
Head direction also outperforms other body directions such as neck or pelvis direction (Table \ref{tab:body_directions}).
These results are significant since they verify that our method can be applied to general VR/AR devices (with or without eye gaze) to enable various motion-related applications.

\paragraph{Short-term vs. Long-term Motion Forecasting}
Prior works in human motion forecasting~\cite{ma2022progressively, mao2021multi} usually classified the motion forecasting task into short-term forecasting (less than $400$ ms) and long-term forecasting (more than $400$ ms).
From the results in Table \ref{tab:global} and Table \ref{tab:local}, we can see that our method consistently outperforms prior methods in terms of both short-term and long-term forecasting.
We also find that the performances of all the methods deteriorate significantly with the increase of prediction time, e.g. the MPJPE error of our method increases from $13.5$ mm at $100$ ms to $160.0$ mm at $1000$ ms for global motion forecasting on the MoGaze dataset.
This is a well-known problem in motion forecasting~\cite{ma2022progressively, guo2023back} that all current methods suffer from since these methods only use historical motion information.
Integrating more context information such as user's goal or task into motion forecasting has the potential to alleviate this problem.
%The likely reason for this is that human motions are stochastic by nature~\cite{barquero2023belfusion} and the randomness magnifies with the increase of time intervals, making it significantly more difficult to forecast long-term motions than short-term motions.

\paragraph{Global vs. Local Motion Forecasting}
Human local motions refer to egocentric body movements while human global motions contain not only egocentric body movements but also global translation and orientation.
We evaluated our method for both global and local motion forecasting and demonstrated that our method significantly outperforms the state-of-the-art methods on both settings (Table \ref{tab:global} and Table \ref{tab:local}).
By comparing the results in Table \ref{tab:global} and Table \ref{tab:local}, we find that our method achieves higher improvements for global motion forecasting (7.4\% on MoGaze and 6.1\% on GIMO) than local motion forecasting (3.9\% on MoGaze and 3.0\% on GIMO).
The likely reason for this is that human eye gaze is closely linked to not only egocentric body movements but also global translation and orientation (see the example in Figure 1) and thus brings more improvements for global motion forecasting.

\paragraph{Limitations}
Despite all the advances that we have made, we identified several limitations that we plan to address in future work.
First, similar to prior methods, our method's long-term motion forecasting performances are not as good as its short-term performances.
Accurately forecasting human motions in long-term period remains a big challenge.
In addition, our method's improvements over the state of the art in local motion forecasting are not as high as in global motion forecasting.
How to enhance the effectiveness of eye gaze in local motion forecasting setting remains to be explored.
Finally, our method takes observed past motions and eye gaze as input while in real applications the input data may be incomplete due to tracking errors and may degrade the performance of our method.
How to deal with incomplete observations is worthy of further study.

\paragraph{Future work}
Besides overcoming the above limitations, many potential avenues of future work exist.
First, it would be interesting to integrate information on 3D environments into our pipeline to improve our method's performance.
In addition, we are also looking forward to adding some physical constraints for the predicted human poses to make them more physically plausible.
Furthermore, integrating our method into motion-related VR/AR applications is an interesting avenue of future work.
Finally, exploring eye-body coordination for other important VR/AR tasks such as cognitive load estimation~\cite{bozkir2019person} and cybersickness prediction or reduction~\cite{lin2022Intentional} is of great significance for VR/AR research.







